T-KAER: Transparency-enhanced Knowledge-Augmented Entity Resolution Framework

Entity resolution (ER) is the process of determining whether two representations refer to the same real-world entity and plays a crucial role in data curation and data cleaning. Recent studies have introduced the KAER framework, aiming to improve pre-trained language models by augmenting external knowledge. However, identifying and documenting the external knowledge that is being augmented and understanding its contribution to the model's predictions have received little to no attention in the research community. This paper addresses this gap by introducing T-KAER, the Transparency-enhanced Knowledge-Augmented Entity Resolution framework. To enhance transparency, three Transparency-related Questions (T-Qs) have been proposed: T-Q(1): What is the experimental process for matching results based on data inputs? T-Q(2): Which semantic information does KAER augment in the raw data inputs? T-Q(3): Which semantic information of the augmented data inputs influences the predictions? To address the T-Qs, T-KAER is designed to improve transparency by documenting the entity resolution processes in log files. In experiments, a citation dataset is used to demonstrate the transparency components of T-KAER. This demonstration showcases how T-KAER facilitates error analysis from both quantitative and qualitative perspectives, providing evidence on "what" semantic information is augmented and "why" the augmented knowledge influences predictions differently.

==> Makefile <==
NAME  = dccpaper
SHELL = bash
PWD   = $(shell pwd)
TEMP := $(shell mktemp -d -t tmp.XXXXXXXXXX)
TDIR  = $(TEMP)/$(NAME)
VERS  = $(shell ltxfileinfo -v $(NAME).dtx)
LOCAL = $(shell kpsewhich --var-value TEXMFLOCAL)
UTREE = $(shell kpsewhich --var-value TEXMFHOME)

.PHONY: source clean distclean inst install uninst uninstall zip ctan

all:	$(NAME).pdf clean
	@exit 0

source: $(NAME).dtx
	tex -interaction=batchmode $(NAME).dtx >/dev/null

ijdc-v9.cls ijdc-v14.cls idcc.cls $(NAME)-base.sty $(NAME)-apacite.bib $(NAME)-biblatex.bib README.md: source

$(NAME).pdf: $(NAME).dtx ijdc-v9.cls ijdc-v14.cls $(NAME)-biblatex.bib $(NAME)-by.pdf
	lualatex -recorder -interaction=batchmode $(NAME).dtx >/dev/null
	biber $(NAME)
	lualatex -recorder -interaction=batchmode $(NAME).dtx >/dev/null
	lualatex -recorder -interaction=batchmode $(NAME).dtx >/dev/null
	@echo "Compilation of PDF finished."

apacitetest.pdf: clean $(NAME).dtx ijdc-v9.cls ijdc-v14.cls $(NAME)-apacite.bib $(NAME)-by.pdf
	lualatex -recorder -interaction=batchmode '\newif\ifapacite\input $(NAME).dtx' >/dev/null
	bibtex $(NAME)
	lualatex -recorder -interaction=batchmode '\newif\ifapacite\input $(NAME).dtx' >/dev/null
	lualatex -recorder -interaction=batchmode '\newif\ifapacite\input $(NAME).dtx' >/dev/null
	mv $(NAME).pdf apacitetest.pdf
	$(MAKE) clean
	@echo "Compilation of PDF finished."

clean:
	rm -f $(NAME).{aux,bbl,bcf,blg,fdb_latexmk,fls,glo,gls,hd,idx,ilg,ind,ins,lsttemp,log,markdown.in,markdown.lua,markdown.out,out,run.xml,synctex.gz} $(NAME)-base.doc ijdc-v9.doc idcc.doc
	rm -rf _markdown_$(NAME)

distclean: clean
	rm -f $(NAME).pdf apacitetest.pdf ijdc-v9.cls ijdc-v14.cls idcc.cls $(NAME)-base.sty $(NAME)-{biblatex,apacite}.bib

inst: all
	mkdir -p $(UTREE)/{tex,source,doc}/latex/$(NAME)
	cp $(NAME).dtx $(UTREE)/source/latex/$(NAME)
	cp {ijdc-v9,ijdc-v14,idcc}.cls $(NAME)-base.sty $(NAME)-by.{eps,pdf} $(UTREE)/tex/latex/$(NAME)
	cp $(NAME).pdf $(NAME)-{biblatex,apacite}.bib README.md $(UTREE)/doc/latex/$(NAME)
	mktexlsr
uninst:
	rm -r $(UTREE)/{tex,source,doc}/latex/$(NAME)
	mktexlsr

install: all
	sudo mkdir -p $(LOCAL)/{tex,source,doc}/latex/$(NAME)
	sudo cp $(NAME).dtx $(LOCAL)/source/latex/$(NAME)
	sudo cp {ijdc-v9,ijdc-v14,idcc}.cls $(NAME)-base.sty $(NAME)-by.{eps,pdf} $(LOCAL)/tex/latex/$(NAME)
	sudo cp $(NAME).pdf $(NAME)-{biblatex,apacite}.bib README.md $(LOCAL)/doc/latex/$(NAME)
	mktexlsr
uninstall:
	sudo rm -r $(LOCAL)/{tex,source,doc}/latex/$(NAME)
	mktexlsr

zip: all
	mkdir $(TDIR)
	cp {ijdc-v9,ijdc-v14,idcc}.cls $(NAME)-base.sty $(NAME)-by.{eps,pdf} $(NAME).{dtx,pdf} README.md Makefile $(TDIR)
	cd $(TEMP); zip -Drq $(PWD)/$(NAME)-$(VERS).zip $(NAME)

ctan: all
	mkdir $(TDIR)
	cp $(NAME).{dtx,pdf} $(NAME)-by.{eps,pdf} README.md Makefile $(TDIR)
	cd $(TEMP); zip -Drq $(PWD)/$(NAME)-$(VERS).zip $(NAME)

